Quick-Tune: Quickly Learning Which Pretrained Model to Finetune and How

With the ever-increasing number of pretrained models, machine learning practitioners are continuously faced with which pretrained model to use, and how to finetune it for a new dataset. In this paper, we propose a methodology that jointly searches for the optimal pretrained model and the hyperparameters for finetuning it. Our method transfers knowledge about the performance of many pretrained models with multiple hyperparameter configurations on a series of datasets. To this aim, we evaluated over 20k hyperparameter configurations for finetuning 24 pretrained image classification models on 87 datasets to generate a large-scale meta-dataset. We meta-learn a multi-fidelity performance predictor on the learning curves of this meta-dataset and use it for fast hyperparameter optimization on new datasets. We empirically demonstrate that our resulting approach can quickly select an accurate pretrained model for a new dataset together with its optimal hyperparameters.

==> Tables/gray-black-box-comparison.tex <==
\begin{table}[]
\centering
\begin{tabular}{lccc}
\toprule
                 & \textbf{Micro} & \textbf{Mini}  & \textbf{Extended} \\
\midrule
\textbf{Black-Box (secs)} & 3491  & 8367  & 31689    \\
\textbf{Gray-Box (secs)}  & 825   & 5441  & 7720     \\
\textbf{Speed-up}         & x4,23 & x1,53 & x4,12   \\
\bottomrule
\end{tabular}
\end{table}



==> Tables/vs_default2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]

\caption{Results in Experiment 1}
\resizebox{\textwidth}{!}{

\begin{tabular}{ccccccc}
\toprule
\multirow{2}{*}{}         & \multicolumn{3}{c}{\textbf{Accuracy}}                                                     & \multicolumn{3}{c}{\textbf{Rank}}                                                            \\ \cmidrule(lr){2-4}\cmidrule(lr){5-7}
                          & \multicolumn{1}{c}{\textbf{Micro}} & \multicolumn{1}{c}{\textbf{Mini}} & \multicolumn{1}{c}{\textbf{Extended}} & \multicolumn{1}{c}{\textbf{Micro}} & \multicolumn{1}{c}{\textbf{Mini}} & \multicolumn{1}{c}{\textbf{Extended}} \\ \midrule
\textbf{Top Model}    & 69.8 $\pm$  24.6    &          63.2   $\pm$    28.7           & 72.0 $\pm$ 20.2                          & 3.56 $\pm$ 0.83                        & 3.61     $\pm$ 1.02                   &          4.13 $\pm$    0.51               \\
\textbf{Middle Model }& 70.5 $\pm$  23.7                      &     62.1 $\pm$ 28.0                & 74.4 $\pm$ 19.9                            & 3.47   $\pm$ 0.76                      & 3.69   $\pm$ 0.57                     & 3.47 $\pm$    0.93                        \\
\textbf{Bottom Model} & 66.9 $\pm$    22.7                     &     59.3 $\pm$   28.7                      & 72.6 $\pm$ 20.1                            & 4.04    $\pm$ 0.79                     & 4.13    $\pm$  0.53                    &  3.97             $\pm$    0.68           \\
\textbf{Quick-Tune}                & \textbf{76.5 $\pm$ 19.7}                        &       \textbf{74.0 $\pm$ 27.6}                  & \textbf{0.051_{ $\pm$ 0.026} }                            & \textbf{2.81     $\pm$ 1.09 }                   & \textbf{2.49   $\pm$  1.18 }              & \textbf{2.29 $\pm$ 0.92 }                            \\ \bottomrule
%\textbf{Oracle }                   & \textbf{89.1 $\pm$   14.3}                &      \textbf{84.2 $\pm$ 16.6}                   & \textbf{91.6 $\pm$ 10.4}                            & \textbf{1.10 $\pm$ 0.41}                         & \textbf{1.05  $\pm$ 0.16}                      & \textbf{1.11 $\pm$ 0.34}                 
\label{tab:experiment1}
\end{tabular}}
\end{table}

==> Tables/vs_models.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\resizebox{\textwidth}{!}{
\begin{tabular}{ccccccc}
\toprule
\multirow{2}{*}{}         & \multicolumn{3}{c}{\textbf{Accuracy}}                                                     & \multicolumn{3}{c}{\textbf{Rank}}                                                            \\ \cmidrule(lr){2-4}\cmidrule(lr){5-7}
                          & \multicolumn{1}{c}{\textbf{Micro}} & \multicolumn{1}{c}{\textbf{Mini}} & \multicolumn{1}{c}{\textbf{Extended}} & \multicolumn{1}{c}{\textbf{Micro}} & \multicolumn{1}{c}{\textbf{Mini}} & \multicolumn{1}{c}{\textbf{Extended}} \\ \midrule
\textbf{Dino} & 70.9 $\pm$ 30.3   & 54.4 $\pm$ 35.5 & 69.5 $\pm$ 25.3 & & &    \\
\textbf{Dino }$\mathbf{\times 2}$ & 72.8 $\pm$ 29.5 &  57.6 $\pm$ 34.0&  71.8 $\pm$ 25.5& &  &\\
\textbf{Dino }$\mathbf{\times 4}$ & 74.7 $\pm$ 28.5 & 61.6 $\pm$ 33.9&  74.5 $\pm$ 24.2& & &\\
\textbf{Dino (unrestricted)} & \textbf{84.5 $\pm$ 21.3} & \textbf{76.5 $\pm$ 28.7} & \textbf{89.1 $\pm$ 13.0} & & &     \\
\textbf{Quick-Tune}      & \underline{76.5 $\pm$ 19.7}   &       \underline{74.0 $\pm$ 27.6}   & \underline{87.5 $\pm$ 11.1} & &  &       \\ 

\bottomrule
\end{tabular}
}
\end{table}

==> Text/2_Motivation.tex <==
\section{Motivation}

%\begin{figure}
%  \begin{center}
%  \end{center}
%   \includegraphics[width=1\linewidth]{Figures/model_vs_dataset_all.pdf}
%  \caption{No silver bullet model: Ranking of models per dataset on the 3 meta-dataset version from Meta-Album~\citep{meta-album-2022}. Models are ordered by size (largest model with index = 0).}
%  \label{fig:ranking_model_vs_dataset}
%\end{figure}


\begin{wrapfigure}{r}{0.36\textwidth}
\vspace*{-1.0cm} 
  \begin{center}
    \includegraphics[width=0.35\textwidth]{Figures/cost-motivation2.pdf}
  \end{center}
  \caption{Error rate of pipelines with different model sizes and learning rates.}
    \label{fig:cost_motivation}
\end{wrapfigure}

Before introducing our method, we present the set of premises that motivated its design choices, aiming for efficient fine-tuning of Deep Learning pipelines. We dubb \textit{pipeline} the combination of model and hyperparmeters to select. In our discussion, we are assuming an efficient set-up, i.e. where time budget and computing resources are limited. The insights depicted in this section are obtained by using our own generated meta-dataset. An extended discussion on the illustration of our motivation is presented in Appendix \ref{app:motivation}.


\textbf{Premise 1:} \textit{There is no silver bullet pretrained model.} Therefore, we need an efficient model hub and a method to select a suitable model for every dataset. In Figure \ref{fig:model_hub_motivation}, we showcase that, given a pool of models, their performance rank varies across datasets.

\textbf{Premise 2:} \textit{The performance during the first epochs is correlated with the performance in last epochs for a given pipeline configuration.} This aspect is the core idea of \textit{Gray-box optimization}~\citep{hutter-book19a}, which leverages this aspect of the learning curves, by training a pipeline only one epoch, without fitting the pipeline until convergence. This also occurs in learning curves observed during finetuning as we demonstrate in Appendix \ref{app:motivating_gray_box}.


\textbf{Premise 3:} \textit{When searching efficient pipelines, we need to account for the cost.} If we balance cost vs. performance, we can encounter high-performing pipelines with less time budget. To exemplify this idea, we compute the error of five different model sizes with five learning rates. In Figure \ref{fig:cost_motivation}, we observe that the optimal pipeline contains a relatively cheap model with 3M parameters.

%\textbf{Premise 2:} \textit{The performance of pipelines with small models is informative about the performance of pipelines with large models.} Thus, we can explore the search space more efficiently by accounting for the \textit{cost} of the pipelines to evaluate, and trading-off this with their performance. To exemplify this idea, we compute the error of five different model sizes with five learning rates. In Figure \ref{fig:cost_motivation}, we observe that the optimal pipeline is in the range of 3M. we observe that the learning rate has a similar effect across model sizes. This idea was also explored in previous work in the context of standard Machine Learning pipelines~\citep{Yang2019_Oboe}.

\textbf{Premise 4:} \textit{Similar datasets have similar performance on the same pipeline configurations.} To leverage this observation, we use \textit{meta-learning} to transfer the knowledge of similar tasks, thus speeding up the optimization.  Previous work has demonstrated its usefulness in general Deep learning tasks~\citep{arango2023deep,ferreira-icml22a}. We illustrate how this also holds for finetuning tasks in Appendix \ref{app:motivating_meta_learning}.




==> Text/4_Preliminaries.tex <==
\section{Preliminaries}

Problem definition of the multi-fidelity, transfer, cost-aware HPO.
\begin{itemize}
    \item Explain multifidelity problem
    \item Introduce the cost-ware component
    \item Introduce the transfer component
\end{itemize}



==> Text/8_Results.tex <==
- Discuss results of experiment 1


==> Text/deprecated-proposed-method.tex <==

\section{Preliminaries}

\textbf{Time-Constrained Automated Finetuning.} We cast automated finetuning as an instance of a Combined Algorithm Selection and Hyperparameter Optimization (CASH)~\citep{thornton-kdd13a} problem. We are given a model hub $\mathcal{B}= \{\beta_1, ..., \beta_M\}$ and a search space of finetuning hyperparameter configurations $\mathbf{x} \in \mathcal{X}$. We refer to the combination of a pretrained model and the fully specified finetuning approach along with its hyperparameters as a deep learning \emph{pipeline} $p:=\left(\mathbf{x}, \beta \right) \in \mathcal{X} \times \mathcal{B}$. The objective is to find the optimal pipeline $p^{*}$ consisting of the optimal pretrained model $\beta^*$ and the associated optimal hyperparameters $\mathbf{x}^*$, which minimize the validation loss $\ell^{(\text{val})}$. The actual parameters $\theta$ of the network $\beta$ that are optimized on the training loss $\ell^{(\text{train})}$ using hyperparameters $\mathbf{x}$ are denoted as $\theta_{\mathbf{x}, \beta}$. The CASH objective function for jointly searching the pipelines is the following bilevel optimization:

%In addition, we have a time budget for search as $ \mathcal{C}(\mathcal{X},\mathcal{B},D) \leq T$. 

\begin{align}
    \label{eq:bilevel}
    p^{*} = (\mathbf{x}^{*}, \beta^*) &\in \argmin_{\mathbf{x} \in \mathcal{X}, \beta \in \mathcal{B}} \;\; \ell^{(\text{val})}\left(\mathbf{x}, \theta^{*}_{\mathbf{x}, \beta} \right), \;\;\; \text{s.t.} \;\;\; \theta^{*}_{\mathbf{x}, \beta} \in \argmin\limits_{\theta} \; \ell^{(\text{train})}\left(\mathbf{x}, \theta_{\mathbf{x}, \beta} \right)
\end{align}

Usually, a policy $\pi$ is used for solving this optimization. Time-constrained scenarios arise when we limit the policy to fit a specific budget $T$, such that the time required by $\pi$ is $t\left( \pi, \mathcal{X}, \mathcal{B} \right) \leq T$. 
%Common policies are Bayesian Optimization or Evolutionary Algorithms.

\textbf{Multi-fidelity Gaussian Processes with Deep Kernels.} Gray-Box HPO~\citep{wistuba2022supervising} exploits partial evaluations $\ell^{(\text{val})}(p, b)$, which represents $\ell^{(\text{val})}\left(\mathbf{x}, \theta^{*}_{\mathbf{x}, \beta} \right)$ after training the weights $\theta$ for $b$ epochs. Our method resembles prior work that builds a probabilistic loss predictor~\cite{wistuba2022supervising}, i.e. surrogate, by feeding the loss curve $\ell^{(\text{val})}(p, i), \forall i=1,\dots,b$ and the pipeline $p \in \mathcal{X} \times \mathcal{B}$ to a multi-layer perceptron (MLP) $\phi: \mathcal{X} \times \mathcal{B} \times \mathrm{R}^{b} \rightarrow \mathrm{R}^Z$. The latent representation $\mathrm{R}^Z$ is coupled with a Gaussian process to yield a deep-kernel covariance component $\mathbf{K}_{p, p'}\left(p, \ell^{(\text{val})}(p, b);  p', \ell^{(\text{val})}(p', b')\right)=\mathbf{K}_{p,p'}\left( \phi\left(p, \ell^{(\text{val})}(p, b) \right),  \phi\left(p', \ell^{(\text{val})}(p', b') \right)\right)$. A Gaussian process estimates the validation loss of a test pipeline as $\ell^{(\text{val})}_* = \ell^{(\text{val})}(p_{*}, b_{*})$ where the asterisk denotes a test pipeline $\left(p_{*}, b_{*}\right)$. Moreover, when $\mathbf{K}_*$ computes the covariance between the training and testing instances, $\mathbf{K}$ is the covariance between training instances, $\mathbf{K}_{**}$ is the covariance between the test instances, and $\ell^{(\text{val})}$ the evaluated training pipelines, then the posterior of the Gaussian process is formalized as:

\begin{equation}
\label{eq:posterior}
    \mathbb{E}\left[\ell^{(\text{val})}_* \mid \mathbf{X}, \mathbf{y}, \mathbf{X}_*\right]=\mathbf{K}_*^T \mathbf{K}_n^{-1} \ell^{(\text{val})}, \;\; \operatorname{cov}\left[\ell^{(\text{val})}_* \mid \mathbf{X}, \mathbf{X}_*\right]=\mathbf{K}_{* *}-\mathbf{K}_*^T \mathbf{K}_n^{-1} \mathbf{K}_*
\end{equation}

This probabilistic output is used subsequently on a multi-fidelity acquisition function for exploring the search space via Bayesian Optimization~\cite{garnett-book22a} given a history of observed learning curves. In this paper, we use the multi-fidelity Expected Improvement~\cite{wistuba2022supervising} as our acquisition function.

%$\mathcal{H}=\left\{\left(\left(x_n, \beta_n, b_n\right), \ell^{(\text{val})}(x_n, \beta_n, b_n)\right)\right\}_{n=1}^N$. 

%\begin{align}
%\mathrm{EI}_{\mathrm{MF}}(\mathbf{x}, \beta, b \mid \mathcal{H}) &= \mathbb{E}\left[\max \left\{f(\mathbf{x}, b)-y_b^{\max }, 0\right\}\right],
%\\ \nonumber
%y_b^{\max } &= \begin{cases}\max \{y \mid((\mathbf{x},  \beta, \cdot, b), \ell^{(\text{val})}) \in \mathcal{H}\} & \text { if }((\mathbf{x},  \beta, \cdot, b), y) \in \mathcal{H} \\ \max \{\ell^{(\text{val})} \mid(\cdot, \ell^{(\text{val})}) \in \mathcal{H}\} & \text { otherwise }\end{cases}
%\end{align}

%\sebastian{Adapt to our formulation}

%\subsection{Quick Automated finetuning via Gray-Box Optimization}
\section{{\ourmethod}: Quick Automated Finetuning}

\begin{algorithm}[ht]
\SetAlgoLined
\KwIn{Model hub $\mathcal{B}=\{ \beta_1, ..., \beta_H\}$, Search space of hyperparameters $\mathbf{x} \in \mathcal{X}$, meta-dataset of pipeline losses $\mathcal{H}_{\ell}^{(M)}$, meta-datasets of pipeline costs $\mathcal{H}^{(M)}_c$, maximum time budget $T$, new dataset $D$ with the associated meta-features $\mathrm{m}$}
\KwOut{Finetuned model $\beta^*$}
Meta-train once $\hat{\ell}^{(\text{val})}(p,b)$ on $\mathcal{H}^{(M)}_{\ell}$ and  $\hat{c}(p, b)$ on $\mathcal{H}^{(M)}_c$ \;

Initialize epoch counts, observed losses, costs and total time $b(p) =0, \mathcal{H}_{\ell} = \emptyset , \mathcal{H}_c = \emptyset, t=0$ \;

Compute meta-features  $\mathbf{m}$ \;
Select randomly a pipeline $p_i \in \mathcal{X} \times \mathcal{B}$ \;
\While{ $t \leq T$}{
Update epoch count $b_{i}:=b(p_i)$, $b_{i}\leftarrow b_{i}+1$\;
Observe loss and cost $\ell_{i} \leftarrow \ell^{(\text{val})}({p_i,  b_{i})}$, $c_{i} \leftarrow c({p_i,  b_{i}})$\;
Checkpoint weights $\theta_{p_i}$ from pipeline $p_i$\;
Update observations $\mathcal{H}_{\ell} \leftarrow \mathcal{H}_{\ell} \cup \{(p_i, b_{i} , \ell_{i})\}$, $\mathcal{H}_c \leftarrow \mathcal{H}_c \cup \{(p_i, b_{i} , c_{i})\}$\;
Fit $\hat{\ell}^{(\text{val})}(p, b)$ and $\hat{c}(p, b)$ on $\mathcal{H}_{\ell}$ and $\mathcal{H}_c$\;
$p_{i} \leftarrow \argmax _{p \in \mathcal{X} \times \mathcal{B}}  \mathrm{EIpu}_{\mathrm{MF}} \left(p,  \mathbf{m},  b(p)+1 \right)$\;
Update total time costs including overhead $t_{oh}$: $t \leftarrow t + t_{\mathrm{oh}} + c_{i}$ \;

}

Obtain best pipeline:  $p^{*} = (\mathbf{x}^*, \beta^*) \in \argmin_{p_i \in \mathcal{H}} \ell^{(\text{val})}(p_i, b_{i})$ \;
Obtain checkpointed weights of the best pipeline: $\theta_{p^*}$\;
\KwRet{$\beta^*, \theta_{p^*}$}\;
\caption{{\ourmethod} Algorithm}
\label{alg:main_algorithm}
\end{algorithm}

% original algorithm just as a backup
%\begin{algorithm}[ht]
%\SetAlgoLined
%\KwIn{Model hub $\mathcal{B}=\{ \beta_1, ..., \beta_H\}$, Search space of hyperparameters $\mathbf{x} \in \mathcal{X}$, meta-dataset of configuration performances $\mathcal{H}^{(M)}_p$, meta-datasets of configuration costs $\mathcal{H}^{(M)}_c$, maximum time budget $T$, new dataset $D$ with the associated meta-features $\mathrm{m}$}
%\KwOut{Fine-tuned model $\beta^*$}
%Meta-train $\hat{\ell}^{(\text{val})}(\mathbf{x},\beta,b)$ on $\mathcal{H}^{(M)}_p$ and  $\hat{c}(\mathbf{x}, \beta, b)$ on $\mathcal{H}^{(M)}_c$ \;

%Initialize epoch counts, observed performances and total time $b(\mathbf{x}, \beta) =0, \mathcal{H} = \emptyset , t=0$ \;

%Compute meta-features  $\mathbf{m}$ \;
%Select randomly $\mathbf{x}_i \in \mathcal{X}, \beta_j  \in \mathcal{B}$ \;
%\While{ $t \leq T$}{
%Update epoch count $b_{i,j}:=b(\mathbf{x}_i, \beta_j)$, $b_{i,j}\leftarrow b_{i,j}+1$\;
%Observe performance and cost $y_{i,j} \leftarrow \ell^{(\text{val})}({\mathbf{x}_i, \beta_j,  b_{i,j})}$, $c_{i,j} \leftarrow c({\mathbf{x}_i, \beta_j,  b_{i,j}})$ \;
%Update observations $\mathcal{H}_p \leftarrow \mathcal{H}_p \cup \{(\mathbf{x}_i, \beta_j, b_{i,j} , y_{i,j})\}$, $\mathcal{H}_c \leftarrow \mathcal{H}_c \cup \{(\mathbf{x}_i, \beta_j, b_{i,j} , c_{i,j})\}$\;
%Fit $\hat{\ell^{(\text{val})}}(\mathbf{x},\beta, b)$ and $\hat{c}(\mathbf{x}, \beta, b)$ on $\mathcal{H}_p$ and $\mathcal{H}_c$\;
%$\mathbf{x}_i, \beta_j \leftarrow \argmax _{\mathbf{x} \in \mathcal{X}, \beta \in \mathcal{B}}  \mathrm{EIpu}_{\mathrm{MF}} \left(\mathbf{x}, \beta,  \mathbf{m},  b(\mathbf{x}, \beta)+1 \right)$\;
%Update total time costs including overhead $t_{oh}$: $t \leftarrow t + t_{\mathrm{oh}} + c_{i,j}$ \;
%}

%Obtain best configuration:  $\mathbf{x}^*, \beta^* \in \argmin_{(\mathbf{x}_i, \beta_j) \in \mathcal{H}} \ell^{(\text{val})}(\mathbf{x}_i, \beta_j, b_{i,j})$ \;
%\KwRet{$\beta^*$}\;
%\caption{{\ourmethod} Algorithm}
%\label{alg:main_algorithm}
%\end{algorithm}



\subsection{Proposed Method}




We propose using deep multi-fidelity Bayesian optimization surrogates to tackle the time-constrained automated finetuning problem. First, we meta-learn loss and cost predictors $\hat{\ell}(\mathbf{x}, \beta, b), \hat{c}(\mathbf{x},\beta, b)$ by leveraging losses $\mathcal{H}^{(M)}$ and costs $\mathcal{H}^{(M)}_c$ in the meta data. We give details on this meta-training process in the supplementary material in Appendix \ref{sec:meta_training_algorithms}. The loss predictor is a multi-fidelity Deep Kernel GP comprising a neural network $\phi : \mathcal{X} \times \mathcal{B} \times M \times \mathrm{R} \rightarrow \mathrm{R}^{Q} $ that embeds the finetuning hyperparameters $\mathbf{x}$, the model $\beta$, task meta-features $\mathbf{m} \in \mathrm{R}^M$ and the current budget to a latent dimension $\mathbf{z} \in \mathrm{R}^{Q}$, and a Mattern Kernel with parameters $\gamma$. Thus, our proposed GP kernel can be formalized as:

\begin{align}
    \kappa(\mathbf{x}, \beta ,b, \mathbf{x}^{\prime}, \beta^{\prime},b^{\prime}, \mathbf{m}) &= \kappa \left( \phi(\mathbf{x}, \beta ,\mathbf{m},b), \phi(\mathbf{x}^{\prime}, \beta^{\prime}, \mathbf{m} ,b^{\prime})) ; \gamma\right)\\
    \text{s.t. \ } & \phi(\mathbf{x}, \beta ,\mathbf{m}, b) = \phi\left(\left[ \mathbf{x}, b,  \mathbf{m}, \xi\left(  \beta ; w^{(\beta)}\right) , \xi\left( \ell(\mathbf{x},b) ; w^{(\ell)}\right) \right] \right)
\end{align}

where $\xi\left(  \beta ; w^{(\beta)}\right)$ and $\xi\left( \ell(\mathbf{x},b) ; w^{(\ell)}\right)$ are parameterized representations of the model and the loss curve respectively. Given a model hub $\mathcal{B}$, the representation of the models is implemented by categorical embeddings of the list of models~\cite{guo-arxiv16a}. The loss curve representation is output by a convolutional neural network following the practice of previous work~\cite{wistuba2022supervising}. 
Although multi-fidelity leverages quick evaluation in low-cost targeted budgets, such as number of epochs, it is not cost-aware. This limits the ability to select configurations whose costs vary independently of the target budget, such as, e.g., the model size. This means that even when evaluating one epoch at a time for quick search space exploration, cost-agnostic approaches might still end up evaluating expensive responses, such as a large model.  
%\sebastian{this could be in the introduction?}

To add cost awareness, we apply a multi-fidelity Expected Improvement per unit cost ($\mathrm{EIpu}_{\mathrm{MF}}$), using the meta-trained cost predictor $\hat{c}(\cdot)$ as $\mathrm{EIpu}_{\mathrm{MF}}(\mathbf{x}, \beta,  \mathbf{m}, b) = \frac{\mathrm{EI}_{\mathrm{MF}}(\mathbf{x}, \beta,  \mathbf{m},  b)}{\hat{c}(\mathbf{x}, \beta,  \mathbf{m}, b)}$ where $\mathrm{EI}_{\mathrm{MF}}$ is the multi-fidelity Expected Improvement~\cite{wistuba2022supervising}. The cost predictor $\hat{c}:\mathcal{X} \times \mathcal{B} \times M \times \mathrm{R} \rightarrow \mathrm{R}$ has exactly the same architecture as the network $\phi(\cdot)$, but we use a different set of parameters and add a linear layer on top for performing a regression task:

\begin{equation}
    \hat{c}(\mathbf{x}, \beta ,\mathbf{m}, b) = \theta ^T\phi\left(\left[ \mathbf{x}, b,  \mathbf{m}, \xi\left(  \beta ; w^{(\beta,c)}\right) , \xi\left( \ell(\mathbf{x},b) ; w^{(\ell,c)}\right) \right] \right)  + \theta_0
\end{equation}

Based on this acquisition function and the meta-trained predictors, we perform Bayesian Optimization as presented in Algorithm \ref{alg:main_algorithm}. At every step we train just one epoch of the configuration $\mathbf{x}_i, \beta_j, b$ that maximizes $\mathrm{EIpu}_{\mathrm{MF}}(\mathbf{x}, \beta,  b)$. Subsequently, we update both the cost predictor and the loss predictor using the observed values. At the end of each BO step, we add the cost of the observed configuration and the overhead to a total counter $t$. This total counter is used to stop the algorithm when $t \leq T$. We show a detailed diagram of our architecture in Figure \ref{fig:architecture_diagram}.


%\subsection{finetuning New Pre-trained Models}

%\begin{figure}
%    \centering
%    \includegraphics[width=0.5\linewidth]{Figures/placeholder-image.png}
%    \caption{Diagram of {\ourmethod} components}
%    \label{fig:approach_diagram}
%\end{figure}

